Breaking Down Out-of-Distribution Detection: Many Methods Based on OOD Training Data Estimate a Combination of the Same Core Quantities

It is an important problem in trustworthy machine learning to recognize out-of-distribution (OOD) inputs which are inputs unrelated to the in-distribution task. Many out-of-distribution detection methods have been suggested in recent years. The goal of this paper is to recognize common objectives as well as to identify the implicit scoring functions of different OOD detection methods. We focus on the sub-class of methods that use surrogate OOD data during training in order to learn an OOD detection score that generalizes to new unseen out-distributions at test time. We show that binary discrimination between in- and (different) out-distributions is equivalent to several distinct formulations of the OOD detection problem. When trained in a shared fashion with a standard classifier, this binary discriminator reaches an OOD detection performance similar to that of Outlier Exposure. Moreover, we show that the confidence loss which is used by Outlier Exposure has an implicit scoring function which differs in a non-trivial fashion from the theoretically optimal scoring function in the case where training and test out-distribution are the same, which again is similar to the one used when training an Energy-Based OOD detector or when adding a background class. In practice, when trained in exactly the same way, all these methods perform similarly.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table_lambda_80M.tex <==


\begin{table*}[!htbp]
\caption{Effect of varying $\lambda$ during training for OE~\cite{HenMazDie2019}, the $s_3$ scoring function for models with background class and \textsc{Shared Combi $s_3$}. While the differences for CIFAR-10 do not seem to be significant for $0.2 \leq \lambda \leq 2$, larger differences can be observed for CIFAR-100. 
}\label{table:lambda}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.0\textwidth}{lC|C|CCCCCCC|C}
%\toprule
\multicolumn{11}{c}{in-distribution: CIFAR-10} \\
\midrule
% Model       & Acc. &  Mean &     SVHN    &   LSUN    &   Uni &   Smooth     &   C-100 & OpenIm  &   CelA  &   80M      \\ 
       & &  Mean &     SVHN    &   LSUN    &   Uni &   Smooth     &   C-100 & OpenIm  &   CelA  &   80M      \\ 
Model    & Acc. &  AUC &    AUC    &   AUC    &   AUC &  AUC    &   AUC & AUC &   AUC &   AUC      \\ \midrule
OE $\lambda = 0.1$
 &  94.89
 &  97.06  
 &  99.08  
 &  98.75  
 &  99.79  
 &  99.95  
 &  93.29  
 &  89.14  
 &  99.46  
 &  97.45   \\
OE $\lambda = 0.2$
 &  95.83
 &  97.53  
 &  99.49  
 &  99.43  
 &  99.83  
 &  99.66  
 &  94.48  
 &  90.13  
 &  99.70  
 &  98.29   \\
OE $\lambda = 0.5$
 &  95.74
 &  97.64
 &  99.48  
 &  99.48  
 &  99.46  
 &  99.64  
 &  94.80  
 &  90.91  
 &  99.71  
 &  98.50 \\
OE $\lambda = 1.0$
 &  95.87
 &  97.73  
 &  99.54  
 &  99.53  
 &  99.70  
 &  99.16  
 &  95.17  
 &  91.36  
 &  99.66  
 &  98.66   \\
OE $\lambda = 2.0$
 &  95.34
 &  97.69  
 &  99.60  
 &  99.37  
 &  99.36  
 &  99.81  
 &  94.79  
 &  91.32  
 &  99.57  
 &  98.54   \\
OE $\lambda = 4.0$
 &  95.31
 &  97.61  
 &  99.51  
 &  99.47  
 &  98.28  
 &  99.72  
 &  95.13  
 &  91.60  
 &  99.56  
 &  98.64   
%  \\[2mm]
% OE $\mu_\lambda$
%  &  95.50
%  &  97.54  
%  &  99.45  
%  &  99.34  
%  &  99.40  
%  &  99.66  
%  &  94.61  
%  &  90.74  
%  &  99.61  
%  &  98.34   \\
%  OE $\sigma_\lambda$
%  &  0.35
%  &  \phantom{0}0.40  
%  &  \phantom{0}0.17  
%  &  \phantom{0}0.27  
%  &  \phantom{0}0.53  
%  &  \phantom{0}0.25  
%  &  \phantom{0}0.63  
%  &  \phantom{0}0.86  
%  &  \phantom{0}0.09  
%  &  \phantom{0}0.42   
 \\
\midrule
\backgroundSthree \  $\lambda=0.1$
 &  95.34 
 &  98.02  
 &  99.70  
 &  99.68  
 &  99.96  
 &  99.97  
 &  95.11  
 &  91.91  
 &  99.83  
 &  98.80   \\
\backgroundSthree \  $\lambda=0.2$
 &  95.46 
 &  98.05  
 &  99.84  
 &  99.61  
 &  99.99  
 &  99.94  
 &  95.10  
 &  92.04  
 &  99.86  
 &  98.82   \\
\backgroundSthree \  $\lambda=0.5$
 &  95.96 
 &  97.98  
 &  99.77  
 &  99.66  
 &  99.32  
 &  99.99  
 &  95.24  
 &  92.01  
 &  99.85  
 &  98.77   \\
\backgroundSthree \  $\lambda=1.0$
 &  95.63
 &  97.96  
 &  99.60  
 &  99.53  
 &  99.97  
 &  99.98  
 &  95.00  
 &  91.70  
 &  99.92  
 &  98.66   \\
\backgroundSthree \  $\lambda=2.0$
 &  95.69  
 &  97.83  
 &  99.40  
 &  99.49  
 &  99.91  
 &  99.96  
 &  94.88  
 &  91.39  
 &  99.80  
 &  98.62   \\
\backgroundSthree \  $\lambda=4.0$
 &  95.25 
 &  97.75  
 &  99.72  
 &  99.38  
 &  99.78  
 &  99.99  
 &  94.31  
 &  91.25  
 &  99.81  
 &  98.29   
%  \\[2mm]
% \backgroundSthree \  $\mu_\lambda$
%  &  95.56 
%  &  97.93  
%  &  99.67  
%  &  99.56  
%  &  99.82  
%  &  99.97  
%  &  94.94  
%  &  91.72  
%  &  99.84  
%  &  98.66   \\
% \backgroundSthree \  $\sigma_\lambda$
%  &   \phantom{0}0.24
%  &  \phantom{0}0.16  
%  &  \phantom{0}0.14  
%  &  \phantom{0}0.10  
%  &  \phantom{0}0.24  
%  &  \phantom{0}0.02  
%  &  \phantom{0}0.30  
%  &  \phantom{0}0.31  
%  &  \phantom{0}0.04  
%  &  \phantom{0}0.18   
 \\
 \midrule
SC $s_3$ \ $\lambda = 0.1$
 &  95.32 
 &  97.59  
 &  99.64  
 &  99.49  
 &  99.94  
 &  99.95  
 &  94.27  
 &  90.11  
 &  99.75  
 &  98.14   \\
SC $s_3$ \ $\lambda = 0.2$
 &  95.56  
 &  97.79  
 &  99.62  
 &  99.57  
 &  99.82  
 &  99.97  
 &  94.59  
 &  91.12  
 &  99.83  
 &  98.39   \\
SC $s_3$ \ $\lambda = 0.5$
 &  95.26 
 &  97.67  
 &  99.41  
 &  99.41  
 &  99.55  
 &  99.82  
 &  94.67  
 &  91.07  
 &  99.75  
 &  98.41   \\
SC $s_3$ \ $\lambda = 1.0$
 &  96.08 
 &  97.96  
 &  99.73  
 &  99.58  
 &  99.95  
 &  99.96  
 &  95.14  
 &  91.48  
 &  99.85  
 &  98.73   \\
SC $s_3$ \ $\lambda = 2.0$
 &  95.74 
 &  97.84  
 &  99.72  
 &  99.60  
 &  99.06  
 &  99.99  
 &  95.15  
 &  91.51  
 &  99.86  
 &  98.77   \\
SC $s_3$ \ $\lambda = 4.0$
 &  95.10 
 &  97.89  
 &  99.84  
 &  99.50  
 &  99.95  
 &  99.94  
 &  94.88  
 &  91.34  
 &  99.78  
 &  98.63   
%  \\[2mm]
% SC $s_3$ \ $\mu_\lambda$ 
%  &  95.51 
%  &  97.79  
%  &  99.66  
%  &  99.52  
%  &  99.71  
%  &  99.94  
%  &  94.78  
%  &  91.10  
%  &  99.80  
%  &  98.51   \\
% SC $s_3$ \ $\sigma_\lambda$
%  &  \phantom{0}0.33 
%  &  \phantom{0}0.20  
%  &  \phantom{0}0.13  
%  &  \phantom{0}0.06  
%  &  \phantom{0}0.32  
%  &  \phantom{0}0.05  
%  &  \phantom{0}0.31  
%  &  \phantom{0}0.47  
%  &  \phantom{0}0.05  
%  &  \phantom{0}0.22   
 \\
 \toprule
\\
\multicolumn{11}{c}{in-distribution: CIFAR-100} \\
\midrule
% Model       &  Acc. &  Mean &       SVHN    &   LSUN      &   Uni &   Smooth    &   C-10 & OpenIm  &   \textcolor{white}{CelA} &   80M      \\ 
       & &  Mean &     SVHN    &   LSUN    &   Uni &   Smooth     &   C-10 & OpenIm  &    &   80M      \\ 
Model    & Acc. &  AUC &    AUC    &   AUC    &   AUC &  AUC    &   AUC & AUC &    &   AUC      \\ 
\midrule
OE $\lambda = 0.1$
 &  76.20
 &  89.13  
 &  86.64  
 &  93.27  
 &  98.21  
 &  99.24  
 &  77.12  
 &  80.32  
 &    
 &  86.13   \\
OE $\lambda = 0.2$
 &  76.99  
 &  81.81  
 &  92.72  
 &  94.25  
 &  48.63  
 &  94.87  
 &  78.50  
 &  81.91  
 &   
 &  87.17   \\
OE $\lambda = 0.5$
 &  76.73
 &  91.72
 &  94.06  
 &  95.58  
 &  99.06  
 &  98.84  
 &  79.53  
 &  83.31 
 &   
 &  88.43 \\
OE $\lambda = 1.0$
 &  75.85 
 &  92.25  
 &  95.05  
 &  96.04  
 &  99.90  
 &  99.36  
 &  79.39  
 &  83.78  
 &   
 &  88.64   \\
OE $\lambda = 2.0$
 &  77.35 
 &  92.60  
 &  95.49  
 &  96.05  
 &  99.59  
 &  99.42  
 &  80.83  
 &  84.24  
 &  
 &  89.16   \\
OE $\lambda = 4.0$
 &  76.49 
 &  92.56  
 &  95.62  
 &  96.09  
 &  99.70  
 &  99.01  
 &  80.39  
 &  84.52  
 &   
 &  89.42   
%  \\[2mm]
% OE $\mu_\lambda$
%  &  76.60
%  &  90.01  
%  &  93.26  
%  &  95.21  
%  &  90.85  
%  &  98.46  
%  &  79.29  
%  &  83.01  
%  &    
%  &  88.16   \\
% OE $\sigma_\lambda$
%  &  0.49
%  &  \phantom{0}4.57  
%  &  \phantom{0}3.12  
%  &  \phantom{0}1.08  
%  &  18.89  
%  &  \phantom{0}1.62  
%  &  \phantom{0}1.22  
%  &  \phantom{0}1.47  
%  &    
%  &  \phantom{0}1.15   
 \\
\midrule
\backgroundSthree \ $\lambda = 0.1$
 &  73.06 
 &  92.35  
 &  94.92  
 &  95.90  
 &  99.94  
 &  99.98  
 &  79.50  
 &  83.87  
 & 
 &  89.19   \\
\backgroundSthree \ $\lambda = 0.2$
 &  75.60 
 &  92.36  
 &  95.46  
 &  95.50  
 &  99.99  
 &  99.83  
 &  79.84  
 &  83.54  
 & 
 &  89.04   \\
\backgroundSthree \ $\lambda = 0.5$
 &  76.42 
 &  92.59  
 &  96.46  
 &  95.57  
 &  99.93  
 &  99.86  
 &  80.01  
 &  83.69  
 & 
 &  88.73   \\
\backgroundSthree \ $\lambda = 1.0$
 &  75.82
 &  91.54  
 &  93.32  
 &  94.64  
 &  99.95  
 &  99.63  
 &  79.29  
 &  82.41  
 & 
 &  88.11   \\
\backgroundSthree \ $\lambda = 2.0$
 &  76.94 
 &  91.67  
 &  93.63  
 &  94.61  
 &  100.00  
 &  99.24  
 &  79.72  
 &  82.83  
 & 
 &  87.95   \\
\backgroundSthree \ $\lambda = 4.0$
 &  76.16 
 &  90.86  
 &  92.18  
 &  93.97  
 &  99.91  
 &  98.23  
 &  79.00  
 &  81.86  
 & 
 &  86.80 
%  \\[2mm]
% \backgroundSthree \ $\mu_\lambda$
%  & 75.67  
%  &  91.90  
%  &  94.33  
%  &  95.03  
%  &  99.95  
%  &  99.46  
%  &  79.56  
%  &  83.03  
%  & 
%  &  88.30   \\
% \backgroundSthree \ $\sigma_\lambda$
%  &  \phantom{0} 1.24 
%  &  \phantom{0}0.63  
%  &  \phantom{0}1.43  
%  &  \phantom{0}0.67  
%  &  \phantom{0}0.03  
%  &  \phantom{0}0.60  
%  &  \phantom{0}0.34  
%  &  \phantom{0}0.73  
%  & 
%  &  \phantom{0}0.81   
 \\
 \midrule
SC $s_3$ \ $\lambda=0.1$
 &  76.12 
 &  89.65  
 &  90.85  
 &  93.62  
 &  99.91  
 &  96.56  
 &  76.71  
 &  80.29  
 &   
 &  86.20   \\
SC $s_3$ \ $\lambda=0.2$
 &  75.68 
 &  90.25  
 &  95.17  
 &  94.31  
 &  93.63  
 &  99.95  
 &  77.23  
 &  81.21  
 &  
 &  87.46   \\
SC $s_3$ \ $\lambda=0.5$
 &  76.11 
 &  91.76  
 &  94.51  
 &  95.27  
 &  99.78  
 &  99.75  
 &  78.73  
 &  82.50  
 &   
 &  88.19   \\
SC $s_3$ \ $\lambda=1.0$
 &  76.52 
 &  92.03  
 &  95.49  
 &  95.42  
 &  99.97  
 &  99.98  
 &  78.46  
 &  82.85 
 &    
 &  88.67   \\
SC $s_3$ \ $\lambda=2.0$
 &  76.67 
 &  92.76  
 &  97.24  
 &  95.82  
 &  100.00  
 &  99.81  
 &  79.89  
 &  83.81  
 &  
 &  89.16   \\
SC $s_3$ \ $\lambda=4.0$
 &  76.25 
 &  92.51  
 &  95.71  
 &  95.58  
 &  99.95  
 &  99.62  
 &  80.31  
 &  83.87  
 &  
 &  89.26   
%  \\[2mm]
% SC $s_3$  \ $\mu_\lambda$
%  &  76.22
%  &  91.49  
%  &  94.83  
%  &  95.00  
%  &  98.87  
%  &  99.28  
%  &  78.56  
%  &  82.42  
%  &  
%  &  88.16   \\
% SC $s_3$  \ $\sigma_\lambda$
%  &   \phantom{0}0.32
%  &  \phantom{0}1.49  
%  &  \phantom{0}1.96  
%  &  \phantom{0}0.78  
%  &  \phantom{0}2.34  
%  &  \phantom{0}1.22  
%  &  \phantom{0}1.30  
%  &  \phantom{0}1.31  
%  &   
%  &  \phantom{0}1.06  
 \\
 \bottomrule
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}







==> table_stats_80M.tex <==
\begin{table*}[!htbp]
\caption{Mean $\mu$ and standard deviation $\sigma$ of the different performance measures over five runs each for models with \textbf{80 Million Tiny Images} as training out-distribution. The training details are the same as for the results shown in Table~\ref{table:80M_sota}.
}\label{table:error}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.0\textwidth}{lC|C|CCCCCCC|C}
%\toprule
\multicolumn{10}{c}{in-distribution: CIFAR-10} \\
\midrule
% Model       & Acc. &  Mean &     SVHN    &   LSUN    &   Uni &   Smooth     &   C-100 & OpenIm  &   CelA  &   80M      \\ 
       & &  Mean &     SVHN    &   LSUN    &   Uni &   Smooth     &   C-100 & OpenIm  &   CelA  &   80M      \\ 
Model    & Acc. &  AUC &    AUC    &   AUC    &   AUC &  AUC    &   AUC & AUC &   AUC &   AUC      \\ \midrule
 Plain $\mu$
 &  94.86
 &  87.72  
 &  92.68  
 &  91.08  
 &  94.11  
 &  81.65  
 &  87.49  
 &  82.50  
 &  84.54  
 &  87.71   \\
  \rowcolor[gray]{.85} Plain $\sigma$
 &  0.12
 &  \phantom{0}3.58  
 &  \phantom{0}1.09  
 &  \phantom{0}0.43  
 &  \phantom{0}4.16  
 &  15.76  
 &  \phantom{0}0.27  
 &  \phantom{0}0.44  
 &  \phantom{0}2.91  
 &  \phantom{0}0.36   \\
 OE~\cite{HenMazDie2019}  $\mu$
 &  95.56
 &  97.70  
 &  99.55  
 &  99.43  
 &  99.79  
 &  99.80  
 &  94.75  
 &  90.85  
 &  99.69  
 &  98.46   \\
  \rowcolor[gray]{.85} OE~\cite{HenMazDie2019} $\sigma$
 &  0.14
 &  \phantom{0}0.10  
 &  \phantom{0}0.07  
 &  \phantom{0}0.08  
 &  \phantom{0}0.18  
 &  \phantom{0}0.11  
 &  \phantom{0}0.10  
 &  \phantom{0}0.12  
 &  \phantom{0}0.02  
 &  \phantom{0}0.08   \\
\midrule
\hspace{\subtab} \backgroundSone $\ \mu$
 &   
 &  96.12  
 &  99.51  
 &  99.25  
 &  99.67  
 &  99.97  
 &  86.62  
 &  88.09  
 &  99.77  
 &  97.89   \\
 \rowcolor[gray]{.85} \hspace{\subtab} \backgroundSone $\ \sigma$
 &   
 &  \phantom{0}0.12  
 &  \phantom{0}0.08  
 &  \phantom{0}0.12  
 &  \phantom{0}0.14  
 &  \phantom{0}0.02  
 &  \phantom{0}0.18  
 &  \phantom{0}0.23  
 &  \phantom{0}0.12  
 &  \phantom{0}0.03   \\
\hspace{\subtab} \backgroundStwo $\ \mu$
 &  95.76 
 &  97.93  
 &  99.67  
 &  99.59  
 &  99.73  
 &  99.96  
 &  95.09  
 &  91.58  
 &  99.87  
 &  98.65   \\
\rowcolor[gray]{.85} \hspace{\subtab} \backgroundStwo $\ \sigma$
 &  \phantom{0}0.18 
 &  \phantom{0}0.12  
 &  \phantom{0}0.07  
 &  \phantom{0}0.06  
 &  \phantom{0}0.34  
 &  \phantom{0}0.04  
 &  \phantom{0}0.05  
 &  \phantom{0}0.23  
 &  \phantom{0}0.04  
 &  \phantom{0}0.03   \\
\backgroundSthree $\ \mu$
 &  95.76 
 &  97.93  
 &  99.67  
 &  99.59  
 &  99.73  
 &  99.96  
 &  95.05  
 &  91.62  
 &  99.87  
 &  98.66   \\
\rowcolor[gray]{.85} \backgroundSthree $\ \sigma$
 &  \phantom{0}0.18 
 &  \phantom{0}0.12  
 &  \phantom{0}0.07  
 &  \phantom{0}0.06  
 &  \phantom{0}0.34  
 &  \phantom{0}0.04  
 &  \phantom{0}0.05  
 &  \phantom{0}0.23  
 &  \phantom{0}0.04  
 &  \phantom{0}0.03   \\
 \midrule
 \hspace{\subtab} Shared BinDisc $\mu$
 &   
 &  97.90  
 &  99.67  
 &  99.63  
 &  99.91  
 &  99.91  
 &  94.60  
 &  91.70  
 &  99.88  
 &  98.74   \\
\rowcolor[gray]{.85}\hspace{\subtab} Shared BinDisc $\sigma$
 &   
 &  \phantom{0}0.10  
 &  \phantom{0}0.13  
 &  \phantom{0}0.04  
 &  \phantom{0}0.07  
 &  \phantom{0}0.12  
 &  \phantom{0}0.14  
 &  \phantom{0}0.16  
 &  \phantom{0}0.02  
 &  \phantom{0}0.03   \\
\hspace{\subtab} Shared Classi $\ \mu$
 &  95.58
 &  95.98  
 &  96.91  
 &  97.54  
 &  99.46  
 &  97.86  
 &  93.08  
 &  88.48  
 &  98.54  
 &  96.21   \\
\rowcolor[gray]{.85}\hspace{\subtab} Shared Classi $\ \sigma$
 &  \phantom{0}0.28
 &  \phantom{0}1.01  
 &  \phantom{0}2.34  
 &  \phantom{0}0.17  
 &  \phantom{0}0.53  
 &  \phantom{0}3.12  
 &  \phantom{0}0.25  
 &  \phantom{0}0.23  
 &  \phantom{0}0.47  
 &  \phantom{0}0.15   \\
Shared \combiStwo $\ \mu$
 &  95.58
 &  97.96  
 &  99.65  
 &  99.62  
 &  99.92  
 &  99.90  
 &  95.02  
 &  91.73  
 &  99.87  
 &  98.70   \\
\rowcolor[gray]{.85}Shared \combiStwo $\ \sigma$
 &  \phantom{0}0.28 
 &  \phantom{0}0.10  
 &  \phantom{0}0.16  
 &  \phantom{0}0.04  
 &  \phantom{0}0.07  
 &  \phantom{0}0.14  
 &  \phantom{0}0.12  
 &  \phantom{0}0.15  
 &  \phantom{0}0.02  
 &  \phantom{0}0.04   \\
Shared \combiSthree $\ \mu$
 &  95.58  
 &  97.95  
 &  99.64  
 &  99.61  
 &  99.92  
 &  99.90  
 &  95.02  
 &  91.72  
 &  99.87  
 &  98.69   \\
\rowcolor[gray]{.85}Shared \combiSthree $\ \sigma$
 &  \phantom{0}0.28 
 &  \phantom{0}0.10  
 &  \phantom{0}0.17  
 &  \phantom{0}0.04  
 &  \phantom{0}0.07  
 &  \phantom{0}0.14  
 &  \phantom{0}0.12  
 &  \phantom{0}0.15  
 &  \phantom{0}0.02  
 &  \phantom{0}0.04   \\
\toprule
\\
\multicolumn{10}{c}{in-distribution: CIFAR-100} \\
\midrule
% Model       &  Acc. &  Mean &       SVHN    &   LSUN      &   Uni &   Smooth    &   C-10 & OpenIm  &   \textcolor{white}{CelA} &   80M      \\ 
       & &  Mean &     SVHN    &   LSUN    &   Uni &   Smooth     &   C-10 & OpenIm  &    &   80M      \\ 
Model    & Acc. &  AUC &    AUC    &   AUC    &   AUC &  AUC    &   AUC & AUC &    &   AUC      \\
  Plain $\mu$
 &  75.95
 &  75.10  
 &  76.89  
 &  77.90  
 &  66.99  
 &  78.90  
 &  75.18  
 &  74.76  
 &   
 &  75.97   \\
  \rowcolor[gray]{.85} Plain $\sigma$
 &  0.19
 &  \phantom{0}6.38  
 &  \phantom{0}3.61  
 &  \phantom{0}0.61  
 &  23.15  
 &  10.26  
 &  \phantom{0}0.35  
 &  \phantom{0}0.29  
 &   
 &  \phantom{0}0.17   \\
 OE~\cite{HenMazDie2019}  $\mu$
 &  76.68
 &  91.56  
 &  93.69  
 &  95.33  
 &  99.38  
 &  99.19  
 &  79.03  
 &  82.76  
 & 
 &  88.08   \\
  \rowcolor[gray]{.85} OE~\cite{HenMazDie2019} $\sigma$
 &  0.55
 &  \phantom{0}0.54  
 &  \phantom{0}1.24  
 &  \phantom{0}0.14  
 &  \phantom{0}0.73  
 &  \phantom{0}0.55  
 &  \phantom{0}0.29  
 &  \phantom{0}0.28  
 &  
 &  \phantom{0}0.28   \\
\midrule

\hspace{\subtab} \backgroundSone $\ \mu$
 &   
 &  78.60  
 &  85.73  
 &  85.59  
 &  98.09  
 &  93.66  
 &  47.51  
 &  61.01  
 &  %85.12  
 &  74.40   \\
\rowcolor[gray]{.85} \hspace{\subtab} \backgroundSone $\ \sigma$
 &   
 &  \phantom{0}3.35  
 &  \phantom{0}5.33  
 &  \phantom{0}1.44  
 &  \phantom{0}3.01  
 &  \phantom{0}8.08  
 &  \phantom{0}0.99  
 &  \phantom{0}1.24  
 & % \phantom{0}1.81  
 &  \phantom{0}0.88   \\
\hspace{\subtab} \backgroundStwo $\ \mu$
 &  76.63 
 &  91.96  
 &  94.42  
 &  95.09  
 &  99.89  
 &  99.79  
 &  79.62  
 &  82.94  
 &  %76.03  
 &  88.39   \\
\rowcolor[gray]{.85} \hspace{\subtab} \backgroundStwo $\ \sigma$
 &  \phantom{0}0.43 
 &  \phantom{0}0.46  
 &  \phantom{0}1.06  
 &  \phantom{0}0.57  
 &  \phantom{0}0.18  
 &  \phantom{0}0.27  
 &  \phantom{0}0.34  
 &  \phantom{0}0.34  
 & % \phantom{0}1.18  
 &  \phantom{0}0.18   \\
\backgroundSthree $\ \mu$
 &  76.63 
 &  91.96  
 &  94.42  
 &  95.09  
 &  99.89  
 &  99.79  
 &  79.62  
 &  82.94  
 &  %76.03  
 &  88.39   \\
\rowcolor[gray]{.85} \backgroundSthree $\ \sigma$
 &  \phantom{0}0.43 
 &  \phantom{0}0.46  
 &  \phantom{0}1.06  
 &  \phantom{0}0.57  
 &  \phantom{0}0.18  
 &  \phantom{0}0.27  
 &  \phantom{0}0.34  
 &  \phantom{0}0.34  
 &  %\phantom{0}1.18  
 &  \phantom{0}0.18   \\
\midrule
 \hspace{\subtab} Shared BinDisc $\mu$
 &   
 &  92.21  
 &  96.63  
 &  95.86  
 &  99.93  
 &  99.97  
 &  77.41  
 &  83.48  
 &  %80.74  
 &  89.19   \\
\rowcolor[gray]{.85}\hspace{\subtab} Shared BinDisc $\sigma$
 &   
 &  \phantom{0}0.34  
 &  \phantom{0}0.91  
 &  \phantom{0}0.30  
 &  \phantom{0}0.08  
 &  \phantom{0}0.02  
 &  \phantom{0}0.51  
 &  \phantom{0}0.23  
 &  %\phantom{0}1.64  
 &  \phantom{0}0.10   \\
\hspace{\subtab} Shared Classi $\ \mu$
 &  76.52
 &  88.31  
 &  88.67  
 &  86.70  
 &  98.97  
 &  99.41  
 &  77.55  
 &  78.59  
 & % 67.39  
 &  82.16   \\
\rowcolor[gray]{.85}\hspace{\subtab} Shared Classi $\ \sigma$
 &  \phantom{0}0.12
 &  \phantom{0}0.89  
 &  \phantom{0}2.33  
 &  \phantom{0}0.64  
 &  \phantom{0}1.04  
 &  \phantom{0}0.48  
 &  \phantom{0}0.50  
 &  \phantom{0}0.34  
 &  %\phantom{0}1.08  
 &  \phantom{0}0.32   \\
Shared \combiStwo $\ \mu$
 &  76.52 
 &  92.34  
 &  96.35  
 &  95.45  
 &  99.95  
 &  99.97  
 &  79.09  
 &  83.23  
 &  %77.22  
 &  88.70   \\
\rowcolor[gray]{.85}Shared \combiStwo $\ \sigma$
 &  \phantom{0}0.12  
 &  \phantom{0}0.34  
 &  \phantom{0}1.01  
 &  \phantom{0}0.24  
 &  \phantom{0}0.05  
 &  \phantom{0}0.02  
 &  \phantom{0}0.48  
 &  \phantom{0}0.25  
 &  %\phantom{0}1.65  
 &  \phantom{0}0.15   \\
Shared \combiSthree $\ \mu$
 &  76.52 
 &  92.33  
 &  96.34  
 &  95.44  
 &  99.95  
 &  99.97  
 &  79.09  
 &  83.22  
 &  %77.16  
 &  88.69   \\
\rowcolor[gray]{.85}Shared \combiSthree $\ \sigma$
 &  \phantom{0}0.12 
 &  \phantom{0}0.34  
 &  \phantom{0}1.02  
 &  \phantom{0}0.24  
 &  \phantom{0}0.05  
 &  \phantom{0}0.02  
 &  \phantom{0}0.48  
 &  \phantom{0}0.25  
 & % \phantom{0}1.64  
 &  \phantom{0}0.15   \\
 \bottomrule
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}






